RNNPose: Recurrent 6-DoF Object Pose Refinement with Robust Correspondence Field Estimation and Pose Optimization

6-DoF object pose estimation from a monocular image is challenging, and a post-refinement procedure is generally needed for high-precision estimation. In this paper, we propose a framework based on a recurrent neural network (RNN) for object pose refinement, which is robust to erroneous initial poses and occlusions. During the recurrent iterations, object pose refinement is formulated as a non-linear least squares problem based on the estimated correspondence field (between a rendered image and the observed image). The problem is then solved by a differentiable Levenberg-Marquardt (LM) algorithm enabling end-to-end training. The correspondence field estimation and pose refinement are conducted alternatively in each iteration to recover the object poses. Furthermore, to improve the robustness to occlusion, we introduce a consistency-check mechanism based on the learned descriptors of the 3D model and observed 2D images, which downweights the unreliable correspondences during pose optimization. Extensive experiments on LINEMOD, Occlusion-LINEMOD, and YCB-Video datasets validate the effectiveness of our method and demonstrate state-of-the-art performance.

==> fig/descrip_loss_knn.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth, trim=0cm 13.5cm 17cm 0cm, clip]{resource/descrip_loss_knn.pdf}
    \vspace{-3ex}
    \caption{ 
    Details about how to identify the correspondences in the 3D model for an observed 2D image point $\mathbf{x}^i$ for 3D-2D descriptor learning. 
    The identified correspondences are used in the descriptor loss $L_{d}$ to construct the positive set $\{~\}_+$ for contrastive leaning. Note that, the ground-truth depth map is rendered according to the ground-truth object pose, and this correspondence identification process is conducted \textbf{only during training}.  
    % Details of the correspondence identification for an arbitrary point of target image. The  descriptors of idendified $K$ correspondences among the model points
    % % of the target image point $\mathbf{x}^i$ 
    % constitute its positive set in the descriptor loss $L_{d}$, and the  
    }
    \label{fig:descrip_loss_knn}
    \vspace{-3ex}
\end{figure}

==> fig/feature_render.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth, trim=0cm 17.5cm 20cm 0cm, clip]{resource/feature_rendering.pdf}
    \vspace{-3ex}
    \caption{ 
        Demonstration of the feature interpolation 
        % during the rasterization  procedure 
        during 3D feature rendering. 
    }
    \label{fig:3D_feature_rendering}
    \vspace{-3ex}
\end{figure}

==> fig/framework_copy.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.99\linewidth, trim=1cm 8.5cm 4cm 1cm, clip]{resource/framework.pdf}
    \vspace{-2ex}
    \caption{
        % The overview of our pose refinement framework. 
        Given an observed image $\mathbf{I}_{obs}$ and an initial object pose $\mathbf{P}_{init}$, RNNPose refines the initial pose to align with the observation recurrently. 
        % an iterative rendering-based pipeline. 
        % Before each refinement, 
        At the beginning, a reference image $\mathbf{I}_{ref}$ is rendered with the object CAD model according to its initial pose $\mathbf{P}_{init}$.   
        % Before the recurrent refinement, 
        Then, the \textbf{Image Feature Encoding} module encodes the rendered reference image and the observed image $\mathbf{I}_{obs}$ as deep feature maps 
        % $\mathbf{F}_{ref}$ and $\mathbf{F}_{obs}$, 
        to establish a pair-wise global correlation volume for lookup later.  
        In parallel, the \textbf{3D Context Feature Encoding} module encodes the 3D model geometry as vertex features which are then rendered with into 2D context feature map $\mathbf{F}_{ctx}$ according to the 
        initial pose to align with $\mathbf{F}_{ref}$, which provides geometric context for the follow-up correspondence estimation. 
        % $\mathbf{F}_{ctx}$ contains shape priors for the follow-up correspondence estimation.
        Based on the prerequisites above, 
        in the \textbf{Pose Refinement} module, the correspondence field $\hat{\mathbf{C}}_t$
        % $\hat{\mathbf{C}}_t$ between $\mathbf{I}_{ref}$ and $\mathbf{I}_{obs}$ is estimated 
        and the residual pose $\delta\hat{\mathbf{P}}_t$ are estimated recurrently in an alternate manner. The pose is optimized by minimizing the Mahalanobis distance between the pose-derived correspondence field $\mathbf{C}(\cdot; \delta\hat{\mathbf{P}}_{t-1})$ and the estimated field $\hat{\mathbf{C}}_t$. 
        % After that, the the residual object pose $\delta\hat{\mathbf{P}}_t$ between $\mathbf{I}_{ref}$ and $\mathbf{I}_{obs}$ is obtained 
        % % estimated by minimizing 
        % by minimizing the Mahalanobis distance between the pose-derived correspondence field $\mathbf{C}(\cdot; \delta\hat{\mathbf{P}}_{t-1})$ and the estimated field $\hat{\mathbf{C}}_t$ via a LM optimizer.
        After the LM pose optimization, $\hat{\mathbf{C}}_t$ is rectified as $\hat{\mathbf{C}}_t'$ with the rigid constraints from the current pose estimation to update the local correlation volumes for next iteration. 
        % the optimized pose rectifies the overall correspondence field as $\hat{\mathbf{C}}_t'$ and also serves as the initial pose for the LM optimization in next RNN iteration. The updated local correlation volume (with $\hat{\mathbf{C}}_t'$) along with $\mathbf{F}_{ctx}$ and $\hat{\mathbf{C}}_t'$ are concatenated as the inputs for next iteration. 
    }
    \label{fig:framework}
    \vspace{-3ex}
\end{figure*}

==> fig/network_arch.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.81\linewidth, trim=0cm 6cm 12cm 0cm, clip]{resource/network_arch_details.pdf}
    % \vspace{-3ex}
    \caption{ 
        Detailed architectures of the networks. 
    }
    \label{fig:network_arch}
    % \vspace{-3ex}
\end{figure*}

==> fig/param_sigma_learning.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\linewidth, trim=0cm 14.5cm 30cm 0cm, clip]{resource/param_sigma_learning.pdf}
    \vspace{-3ex}
    \caption{ The learning process of the parameter $\sigma$ in the similarity score Eq. (3). 
    }
    \label{fig:param_sigma_learning}
    \vspace{-3ex}
\end{figure}

==> fig/pose_vis_full.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.99\linewidth, trim=0cm 0cm 20cm 7.5cm, clip]{resource/pose_vis_full.pdf}
    \vspace{-3ex}
    \caption{ More Visualizations of estimated poses and similarity score maps on Occlusion LINEMOE dataset.
    For pose visualization, the white boxes represent the erroneous initial poses, the red boxes are estimated by our algorithm and the ground-truth boxes are in blue. Here, the initial poses for pose refinement are originally from PVNet~\cite{peng2019pvnet} but added with significant disturbances for robustness testing ( adding Gaussian noise $\sigma_t=0.09$ cm, $\sigma_r=10^\circ$). For the similarity score map, brighter color represents a higher similarity.   
    }
    \label{fig:pose_vis_full}
    % \vspace{-3ex}
\end{figure*}

==> fig/recurrent_refine_vis.tex <==
\begin{figure*}[t!]
    \centering
    % \includegraphics[width=1\linewidth, trim=1cm 1cm 2cm 0cm, clip]{resource/recurrent_refine_vis2.pdf}
    \includegraphics[width=1\linewidth, trim=1cm 2cm 20cm 0cm, clip]{resource/recurrent_refine_vis2.pdf}
    \vspace{-3ex}
    \caption{ 
        Visualizations of the 
        % rendered image, observed image,  
        estimated correspondence fields (CFs), rectified CFs, warped observed image with the CFs and the pose estimation of each recurrent iteration (iter1-iter4) in the first rendering cycle. For pose visualization, the white boxes represent the input erroneous initial poses, the red boxes are estimated by our algorithm, while the ground-truth boxes are in blue.
    % More Visualizations of estimated poses and similarity score maps on Occlusion LINEMOE dataset.
    % For pose visualization, the white boxes represent the erroneous initial poses, the red boxes are estimated by our algorithm and the ground-truth boxes are in blue. Here, the initial poses for pose refinement are originally from PVNet~\cite{peng2019pvnet} but added with significant disturbances for robustness testing ( adding Gaussian noise $\sigma_t=0.09$ cm, $\sigma_r=10^\circ$). For the similarity score map, brighter color represents a higher similarity.   
    }
    \label{fig:recurrent_refine_vis}
    % \vspace{-3ex}
\end{figure*}

==> fig/renreciter.tex <==
\begin{figure}[t!]
    \centering
    \resizebox{0.8\linewidth}{!}{
    \includegraphics[width=1\linewidth, trim=0cm 17.5cm 27cm 0cm, clip]{resource/renreciter.pdf}
    \vspace{-4ex}
    }
    \caption{ 
        The estimation accuracies with different recurrent iterations and rendering iterations on LINEMOD dataset.  The evaluation is based on ADD(-S) metric. (a) Results based on the initial poses from PoseCNN~\cite{xiang2017posecnn}. (b) We further disturb the PoseCNN estimations in (a) by adding Gaussian pose noise ($t_{std}=15$cm, $r_{std}=10^{\circ}$). 
    }
    \label{fig:renreciter}
    \vspace{-3ex}
\end{figure}

==> table/ablation_lmocc.tex <==
\begin{table}[t]
  % \small
  \centering
  \caption{Ablation study on LINEMOD dataset with the ADD(-S) score. The initial poses are provide by PoseCNN for the experiments in this table. }
  \setlength\tabcolsep{4pt}
  % \scalebox{0.8}{
  \resizebox{1\linewidth}{!}{
    % \begin{tabular}{c||ccccc|cc}
    \begin{tabular}{c||ccccccccccccccc|ccc|}
      \hline
      Object      &\multicolumn{3}{c}{w/o flow loss} & \multicolumn{3}{c}{w/o alignment loss} & \multicolumn{3}{c}{w/o $\hat{\mathbf{C}}_t'$ rect.}  & \multicolumn{3}{c}{w/o 3D context $\mathbf{F}_{ctx}$} & \multicolumn{3}{c}{w/ 2D context}& \multicolumn{3}{c}{Full(Ours)}\\\hline
      % Init. Pose  & -       & -       & -             & self-designed   & PVNet         &PoseCNN&PVNet\\ \hline
      Ape         &     &     &           & -               &               &\\
      Can         &     &     &           & -               & \textbf{} &\\
      Cat         &     &     &           & -               & \textbf{} &\\
      Driller     &     &     &           & -               & \textbf{} &\\
      Duck        &     &     &           & -               & \textbf{} &\\
      Eggbox      &     &     &           & -               &           &\\
      Glue        &     &     &          & -                & \textbf{} &\\
      Holep.      &     &     &          & -                &           &\\ \hline
      Average     &     &     &           &             & \textbf{} &\\ \hline
    \end{tabular}
    }
  \label{tab:lmocc}
\end{table}
  

==> table/runtime.tex <==
\begin{table}[t]
    \caption{Runtime analysis of individual modules.}
    \centering
    \resizebox{1\linewidth}{!} {
    \begin{tabular}{c||cccccc}
    \hline
    Module & Runtime (ms) \\
    \hline
    Image Rendering         &8.88                   \\
    3D Feature Rendering    &5.39                   \\
    Image Feature Encoding  &6.39    \\ 
    2D-3D Hybrid Net        &2.99               \\ 
    CF Estimation           &6.21              \\ 
    Pose Optim.             &6.23                \\ 
    CF Rectification        &1.48               \\   
    \hline
    \end{tabular}
    }
    \label{tab:runtime}
\end{table}

% \begin{table}[t]
%     \caption{}
%     \centering
%     \resizebox{1\linewidth}{!} {
%     \begin{tabular}{c||cccccc}
%     \hline
%     & Renderer& Image feature encoding & 2D-3D hybrid& CF estimation  & Pose optim. &  CF rectification \\  \hline %& \multicolumn{1}{c}{CosyPose~\cite{labbe2020}}
%     Runtime &  &  &   & & \\
%     \hline
%     \end{tabular}
%     }
%     \label{tab:runtime}
% \end{table}
